Paraxial fluid of light in hot atomic vapors

Quantum fluids of light are the photonic counterpart of Bose gases. They currently attract increasing interest since they are versatile and highly tunable systems for probing many-body physics quantum phenomena, such as superfluidity. Superfluid flow of light has already been reported in microcavity exciton-polariton condensates but clear observation of this phenomenon in cavityless systems, that is, for propagating photon fluids, remains elusive. In this thesis, we study the hydrodynamical properties of light propagating close to resonance in hot rubidium vapors. Whereas photons in air are not interacting with each other, the situation is different in rubidium vapors, as an effective interaction between them, mediated by the atomic ensemble, appears. The light behaves therefore as a fluid flowing in the plane perpendicular to the optical axis. The primary purpose of this thesis was to show that light in those systems can behave as a superfluid. The first step toward the observation of superfluidity is to measure the dispersion relation of small amplitude density waves travelling onto the propagating photon fluid. I show that this dispersion exhibits a linear trend for small excitation wave-vectors, which is, according to the Landau criterion, a sufficient condition for guaranteeing superfluidity. I present then an all-optical defect experiment - where the photon fluid flows against an optically induced obstacle (namely, a local change of refractive index) - designed to measure the drag force cancellation at the fluid/superfluid threshold.

==> thcoverdata.tex <==
%!TeX encoding = UTF-8
% Metadata for coverpages
\thesisname{Thèse de doctorat}
\gradename{docteur}
\univ{de Sorbonne Université}
\logos{SorbonneUniv}{LKB}{CNRS}                   % Un à trois logo. Le 1er est celui de \univ
\specialite{Physique}
\ecoledoctnum{564}
\ecoledoct{Physique en Île-de-France}
\title{Paraxial fluid of light in hot atomic vapors}
\titleen{Fluide de lumière en géométrie propageante}

% si nécessaire, pour les métadonnées
%\titlemeta{La laine des Dupondt au Pays de l'or noir} 
%\titlemetaen{Dupondt's wool in "Land of Black Gold" } 

\date{31/01/2019}
\author{Quentin FONTAINE}
\advisor{Quentin GLORIEUX}
\atinstitution{à Sorbonne Université}
\atlab{{\Large au Laboratoire Kastler Brossel}}
% Jury as LaTeX Tabular. Pas de président avant soutenance								  
\jury{ %                         
M. & Luis OROZCO & Rapporteur        \\
M. & Iacopo CARUSOTTO & Rapporteur        \\
Mme & Agnès MAÎTRE & Examinatrice           \\
Mme & Claire MICHEL & Examinatrice         \\
Mme & Hélène PERRIN & Examinatrice           \\
M. & Quentin GLORIEUX & Directeur de thèse      \\
M. & Alberto BRAMATI & Co-encadrant}
\makeatletter
\@ifpackageloaded{thcover-psl}{\logos{PSL}{LKB}{}}{\relax}
\makeatother

\resume{Quantum fluids of light are the photonic counterpart of Bose gases. They currently attract increasing interest since they are versatile and highly tunable systems for probing many-body physics quantum phenomena, such as superfluidity. Superfluid flow of light has already been reported in microcavity exciton-polariton condensates but clear observation of this phenomenon in cavityless systems, that is, for propagating photon fluids, remains elusive. 
\vspace{6pt}
\newline
\noindent In this thesis, we study the hydrodynamical properties of light propagating close to resonance in hot rubidium vapors. Whereas photons in air are not interacting with each other, the situation is different in rubidium vapors, as an effective interaction between them, mediated by the atomic ensemble, appears. The light behaves therefore as a fluid flowing in the plane perpendicular to the optical axis. The primary purpose of this thesis was to show that light in those systems can behave as a superfluid. The first step toward the observation of superfluidity is to measure the dispersion relation of small amplitude density waves travelling onto the propagating photon fluid. I show that this dispersion exhibits a linear trend for small excitation wave-vectors, which is, according to the Landau criterion, a sufficient condition for guaranteeing superfluidity. I present then an all-optical defect experiment - where the photon fluid flows against an optically induced obstacle (namely, a local change of refractive index) - designed to measure the drag force cancellation at the fluid/superfluid threshold.}

\motscles{fluid of light, hot rubidium vapors, Bogoliubov dispersion, superfluidity.}

% si nécessaire, pour les métadonnées
%\titlemetaen{Dupondt's wool in "Land of Black Gold" } 

\abstract{Les fluides quantiques de lumière constituent l'analogue$\,$optique$\,$des$\,$condensats de Bose-Einstein atomiques. Ils ont suscité une attention croissante au sein de la communauté scientifique puisqu'ils permettent de sonder facilement des phénomènes quantiques à N-corps, à l'instar de la superfluidité. Des écoulements superfluides de lumière ont déjà été mis en évidence dans des fluides de polaritons en micro-cavité mais les observations rapportées jusqu'à présent dans les fluides de lumière en géométrie propageante sont moins probantes.
\vspace{6pt}
\newline
\noindent Dans cette thèse, nous étudions les propriétés hydrodynamiques de la lumière propageant à quasi-resonance dans une vapeur chaude de rubidium. Alors que les photons n'intéragissent pas entre eux dans l'air, la situation est différente dans la vapeur de rubidium, puisqu'une interaction effective entre photons, médiée par le milieu atomique, apparaît. La lumière peut alors être décrite comme un fluide s'écoulant dans le plan perpendiculaire à l'axe optique. L'objectif premier de cette thèse était de démontrer que la lumière, en propageant dans ce système, peut se comporter comme un superfluide. Dans cette perspéctive, il est nécessaire de mesurer tout d'abord la relation de dispersion à laquelle obéissent les ondes de densité de faible amplitude se déplaçant à la surface du fluide de lumière. Je montre que cette dispersion dépend linéairement du module du vecteur d'onde quand celui-ci est petit devant la longueur de cicatrisation du système ; d'après le critère de Landau, ceci est suffisant pour garantir l'existence d'écoulements superfluides de lumière. Je présente ensuite une expérience visant à mesurer l'annulation de la force de trainée exercée par le fluide de lumière sur un obstacle optique (\textit{ie} un changement local d'indice de réfraction) au passage de la transition fluide/superfluide.´          


% Alors que les photons dans le vide sont des particules qui n'intéragissent pas entre elles,  
}

\keywords{fluide de lumière, vapeur chaude de rubidium, dispersion de Bogoliubov, superfluidité}


